Latch Based Design for Fast Voltage Droop Response

We present a latch-based and PLL-free design of the voltage droop correction circuit of Lenzen, Fuegger, Kinali, and Wiederhake\cite{DroopJournal}. Such a circuit dynamically modifies the clock frequency of a digital clock for VLSI systems. Our circuit responds within two clock cycles and halves the length of the synchroniser chain compared to the previous design. Further, we introduce a differential sensor based design for masking latches as a replacement for masking flip flops that the design of \cite{DroopJournal} requires, but leaves unspecified. The use of latches instead of threshold-altered flip flops alters the timing properties of our design and thus the proofs of correctness that accompanied their design require modifications which we present here. This design has been successfully implemented on the IHP 130 nm process technology. The results of the experimental measurements will be discussed in a subsequent publication.

==> contents/figures/phase_acc_interface.tex <==
\begin{tikzpicture}
    
\end{tikzpicture}
